Computer Vision Self-supervised Learning Methods on Time Series

Self-supervised learning (SSL) has had great success in both computer vision. Most of the current mainstream computer vision SSL frameworks are based on Siamese network architecture. These approaches often rely on cleverly crafted loss functions and training setups to avoid feature collapse. In this study, we evaluate if those computer-vision SSL frameworks are also effective on a different modality (\textit{i.e.,} time series). The effectiveness is experimented and evaluated on the UCR and UEA archives, and we show that the computer vision SSL frameworks can be effective even for time series. In addition, we propose a new method that improves on the recently proposed VICReg method. Our method improves on a \textit{covariance} term proposed in VICReg, and in addition we augment the head of the architecture by an iterative normalization layer that accelerates the convergence of the model.

==> fine_tune_eval_ptb-xl.tex <==
% \begin{linespread}{1.0}
% \begin{table}[H]
% \centering
% \footnotesize
% \addtolength{\leftskip} {-0.6cm}

% \caption{Fine-tuning evaluation on a subset of the PTB-XL, where the subset used for the fine-tuning is the 1st fold. That is, 12.5\% of the training dataset. The results are obtained over 5 runs.}
% \label{table:fine_tune_ev_ptb_xl}

% \begin{tabular}{lccccccc}

% \toprule
% \multicolumn{1}{c}{PTB-XL} & CPC    & SimSiam & Barlow Twins & VICReg & VIbCReg & VbIbCReg & \texttt{Supervised} \\
% \midrule
% Macro AUC                  & 0.8313(30) & 0.8179(120)  & 0.8325(39)  & \textbf{0.8692(25)} & 0.8514(26)  & 0.8506(27)   & \underline{0.8643(12)}     \\
% Valid. loss                & 0.0768(3) & 0.0845(20)  & 0.0802(6)  & 0.0754(3) & \underline{0.0750(2)}  & \textbf{0.0743(1)}   & 0.0765(2)     \\
% Test loss                  & 0.0776(3) & 0.0831(14)  & 0.0792(11)  & \textbf{0.0749(4)} & 0.0764(2)  & \underline{0.0757(2)}   & \textbf{0.0749(3)}     \\
% \bottomrule

% \end{tabular}
% \end{table}
% \end{linespread}




\begin{sidewaystable}
\sidewaystablefn%
\begin{center}
\begin{minipage}{\textheight}

\caption{Fine-tuning evaluation on a subset of the PTB-XL, where the subset used for the fine-tuning is the 1st fold. That is, 12.5\% of the training dataset. The results are obtained over 5 runs.}
\label{table:fine_tune_ev_ptb_xl}

\footnotesize
\begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lcccccccc  c@{\extracolsep{\fill}}}

\toprule%
\multicolumn{1}{c}{PTB-XL} & SimCLR & BYOL & CPC    & SimSiam & Barlow Twins & VICReg & TNC & VIbCReg & \texttt{Supervised} \\
\midrule
Macro AUC     & 0.7853(73) & 0.746(37) & 0.8313(30) & 0.8179(120)  & 0.8325(39)  & \textbf{0.8692(25)} & 0.5368(145) & 0.8514(26)    & \underline{0.8643(12)}     \\
Valid. loss   & 0.081(3) & 0.0842(2) & 0.0768(3) & 0.0845(20)  & 0.0802(6)  & 0.0754(3) & 0.1077(4) & \underline{0.0750(2)}  & \underline{0.0765(2)}     \\
Test loss     & 0.0808(3) & 0.0843(5) & 0.0776(3) & 0.0831(14)  & 0.0792(11)  & \textbf{0.0749(4)} & 0.1066(5) & \underline{0.0764(2)}   & \textbf{0.0749(3)}     \\
\botrule

\end{tabular*}
\end{minipage}
\end{center}
\end{sidewaystable}

==> linear_eval_ptb_xl.tex <==
% \begin{linespread}{1.0}
% \begin{table}[H]
% \centering
% \footnotesize
% \addtolength{\leftskip} {-1.6cm}

% \caption{Linear evaluation on the PTB-XL. The results are obtained over 5 runs. For the PTB-XL, a macro AUC score is commonly used as a linear evaluation score \cite{Strodthoff2020DeepPTB-XL, Mehari2021Self-supervisedData}. Additionally, the lowest validation and test losses are presented to cover an aspect of the evaluation that the macro AUC cannot cover. The validation loss is computed on the 9-th fold in the same setting as the training, and the test loss is computed on the 10-th fold in the same setting as the training except that no augmentation is applied on input data. Note that a binary cross entropy loss for multiple classes is used (\textit{i.e.,} \texttt{BCEWithLogitsLoss} in PyTorch). The standard deviation values within the parentheses are presented, multiplied by 10000 (\textit{i.e.,} 0.0002 $\rightarrow$ 2).}

% \begin{tabular}{lccccccc | c}

% \toprule
% \multicolumn{1}{c}{PTB-XL} & \texttt{Rand Init} & CPC & SimSiam & Barlow Twins & VICReg & \textbf{VIbCReg} & \textbf{VbIbCReg} &
% \texttt{Supervised} \\
% \midrule
% Macro AUC   & 0.4634(137) & 0.8268(20) & 0.5899(356) & 0.7524(224) & 0.8316(11) & \textbf{0.8478(31)} & \underline{0.8444(32)} & 0.9311(18) \\
% Valid. loss & 0.1078(2) & 0.0799(3) & 0.1025(9) & 0.0906(33) & 0.0791(2) & \underline{0.0750(2)} & \textbf{0.0747(2)} & 0.0629(2) \\
% Test loss   & 0.1071(2) & 0.0806(1) & 0.1013(10) & 0.0890(26) & 0.0788(3) & \underline{0.0760(2)} & \textbf{0.0758(2)} & 0.0612(3) \\
% \bottomrule

% \end{tabular}
% \label{table:LE_ptb_xl}
% \end{table}
% \end{linespread}



\begin{sidewaystable}
\sidewaystablefn%
\begin{center}
\begin{minipage}{\textheight}
\caption{Linear evaluation on the PTB-XL. The results are obtained over 5 runs. For the PTB-XL, a macro AUC score is commonly used as a linear evaluation score \cite{Strodthoff2020DeepPTB-XL, Mehari2021Self-supervisedData}. Additionally, the lowest validation and test losses are presented to cover an aspect of the evaluation that the macro AUC cannot cover. The validation loss is computed on the 9-th fold in the same setting as the training, and the test loss is computed on the 10-th fold in the same setting as the training except that no augmentation is applied on input data. Note that a binary cross entropy loss for multiple classes is used (\textit{i.e.,} \texttt{BCEWithLogitsLoss} in PyTorch). The standard deviation values within the parentheses are presented, multiplied by 10000 (\textit{i.e.,} 0.0002 $\rightarrow$ 2).}
\label{table:LE_ptb_xl}
\tiny
\begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lccccccccc c@{\extracolsep{\fill}}}
\toprule%
\multicolumn{1}{c}{PTB-XL} & \texttt{Rand Init} & SimCLR & BYOL & CPC & SimSiam & Barlow Twins & VICReg & TNC & \textbf{VIbCReg} & \texttt{Supervised} \\
\midrule
Macro AUC   & 0.4634(137) & \textbf{0.854(50)} & 0.8321(21) & 0.8268(20) & 0.5899(356) & 0.7524(224) & 0.8316(11) & 0.602(112) & \underline{0.8478(31)}  & 0.9311(18) \\
Valid. loss & 0.1078(2) & \textbf{0.0729(8)} & \underline{0.075(3)} & 0.0799(3) & 0.1025(9) & 0.0906(33)) & 0.0791(2) & 0.1032(1) & \underline{0.0750(2)} & 0.0629(2) \\
Test loss   & 0.1071(2) & \textbf{0.0731(6)} & \underline{0.0756(2)} & 0.0806(1) & 0.1013(10) & 0.0890(26) & 0.0788(3) & 0.1024(2) & {0.0760(2)}  & 0.0612(3) \\
\botrule
\end{tabular*}
\end{minipage}
\end{center}
\end{sidewaystable}
